Low Precision Decentralized Distributed Training over IID and non-IID Data

Decentralized distributed learning is the key to enabling large-scale machine learning (training) on edge devices utilizing private user-generated local data, without relying on the cloud. However, the practical realization of such on-device training is limited by the communication and compute bottleneck. In this paper, we propose and show the convergence of low precision decentralized training that aims to reduce the computational complexity and communication cost of decentralized training. Many feedback-based compression techniques have been proposed in the literature to reduce communication costs. To the best of our knowledge, there is no work that applies and shows compute efficient training techniques such as quantization, pruning, etc., for peer-to-peer decentralized learning setups. Since real-world applications have a significant skew in the data distribution, we design "Range-EvoNorm" as the normalization activation layer which is better suited for low precision training over non-IID data. Moreover, we show that the proposed low precision training can be used in synergy with other communication compression methods decreasing the communication cost further. Our experiments indicate that 8-bit decentralized training has minimal accuracy loss compared to its full precision counterpart even with non-IID data. However, when low precision training is accompanied by communication compression through sparsification we observe a 1-2% drop in accuracy. The proposed low precision decentralized training decreases computational complexity, memory usage, and communication cost by 4x and compute energy by a factor of ~20x, while trading off less than a $1\%$ accuracy for both IID and non-IID data. In particular, with higher skew values, we observe an increase in accuracy (by ~ 0.5%) with low precision training, indicating the regularization effect of the quantization.

==> table_notations.tex <==
\begin{table}[]
    \centering
        \caption{Description for the notations used in the equations.~\ref{eq:bn}} 
    \label{tab:notations}
         
    \begin{minipage}{\linewidth}
     \centering
    \resizebox{\textwidth}{!}{
     \begin{tabular}{|c|c|}
         \hline
        Notation  & Description \\
        \hline
        $B$  & Batch size \\
        \hline
        $C_{in}$  &\# of Input channels \\
        \hline
         $C_{out}$  &\# of Output channels \\
        \hline
        $K$  & Kernel Size for convolution \\
        \hline
        $L$  & Height/Width of input \\
        \hline
        $P$  & Padding for convolution \\
        \hline
        $S$  & Stride for convolution \\
        \hline
         \end{tabular}
        }
    \end{minipage} 
\end{table}
